Quenching star formation with low-luminosity AGN winds

We present a simple model for low-luminosity active galactic nucleus (LLAGN) feedback through winds produced by a hot accretion flow. The wind carries considerable energy and deposits it on the host galaxy at kiloparsec scales and beyond, heating the galactic gas thereby quenching star formation. Our model predicts that the typical LLAGN can quench more than $10\%$ of star formation in its host galaxy. We find that long-lived LLAGN winds from supermassive black holes (SMBH) with masses $\geq 10^8 M_{\odot}$ and mass accretion rates $\dot{M} > 10^{-3} \medd \ (0.002 \msun / yr)$ can prevent gas collapse and significantly quench galactic star formation compared to a scenario without AGN, if the wind persists over 1 Myr. For sustained wind production over timescales of 10 Myr or longer, SMBHs with $10^8 M_{\odot}$ or larger masses have important feedback effects with $\dot{M} > 10^{-4} \medd \ (0.0002 \msun / yr)$.

==> tables.tex <==
\iffalse
\begin{table}
    \centering
    \begin{tabular}{lcc}
        \hline
        $\nu$ (Hz) & $\nu L_{\nu}$ (erg s$^{-1}$) & Reference \\
        \hline
        1.36E+09           & (5.33 $\pm$ 0.20)E+031 & \cite{Falcke1998}       \\
        1.44E+09           & (5.64 $\pm$ 0.21)E+031 & \cite{Falcke1998}       \\
        1.64E+09           & (6.67 $\pm$ 0.36)E+031 & \cite{Falcke1998}       \\
        4.85E+09           & (2.30 $\pm$ 0.04)E+032 & \cite{Falcke1998}       \\
        8.45E+09           & (4.50 $\pm$ 0.06)E+032 & \cite{Falcke1998}       \\
        1.49E+10           & (1.13 $\pm$ 0.03)E+033 & \cite{Falcke1998}       \\
        2.25E+10           & (1.83 $\pm$ 0.08)E+033 & \cite{Falcke1998}       \\
        4.33E+10           & (4.48 $\pm$ 0.45)E+033 & \cite{Falcke1998}       \\
        9.30E+10           & (1.31 $\pm$ 0.34)E+034 & \cite{Falcke1998}       \\
        9.50E+10           & (1.40 $\pm$ 0.28)E+034 & \cite{Falcke1998}       \\
        9.50E+10           & (1.48 $\pm$ 0.16)E+034 & \cite{Falcke1998}       \\
        1.06E+11           & (1.89 $\pm$ 0.28)E+034 & \cite{Falcke1998}       \\
        1.50E+11           & (3.44 $\pm$ 0.44)E+034 & \cite{Falcke1998}       \\
        1.51E+11           & (3.24 $\pm$ 0.23)E+034 & \ci        1.51E+11           & (3.24 $\pm$ 0.23)E+034 & \cite{Falcke1998}       \\

te{Falcke1998}       \\
        1.52E+11           & (3.27 $\pm$ 0.28)E+034 & \cite{Falcke1998}       \\
        2.36E+11           & (4.88 $\pm$ 1.57)E+034 & \cite{Falcke1998}       \\
        8.50E+11           & (4.40 $\pm$ 1.26)E+035 & \cite{Zhao2003}       \\
        1.23E+13           & < 4.56E+035 & \cite{Serabyn1997}       \\
        3.49E+13           & < 2.17E+036 & \cite{Schodel2011}    \\
        6.25E+13           & (1.75 $\pm$ 0.60)E+034 & \cite{Schodel2011}    \\
        7.89E+13           & (2.92 $\pm$ 0.35)E+034 & \cite{Schodel2011}    \\
        1.38E+14           & 1.12E+034 & \cite{Dodds2011} \\
        1.43E+14           & (2.32 $\pm$ 0.21)E+034 & \cite{Meyer2009}      \\
        1.50E+14           & < 2.22E+034 & \cite{Hornstein2002}  \\
        (4.79 -- 23.99)E+17 &           & \cite{Baganoff2003}
        \\
        \hline
    \end{tabular}
    \caption{SED data for SgrA*.}
    \label{tab:M87}
\end{table}
\fi
\begin{table}
    \centering
    \begin{tabular}{lcc}
        \hline
        $\nu$ (Hz) & $\nu L_{\nu}$ (erg s$^{-1}$) & Reference \\
        \hline
        1.60E+09 & 1.87E+038 & \cite{Giovannini1990}\\
        8.40E+09 & 1.41E+039 & \cite{Morabito1986} \\
        2.20E+10 & 2.48E+039 & \cite{Junor1995}    \\
        8.60E+10 & 4.43E+039 & \cite{Lee2008}      \\
        1.00E+11 & 1.61E+040 & \cite{Lonsdale1998} \\
        2.30E+11 & 7.25E+040 & \cite{Doeleman2012} \\
        2.60E+13 & 1.09E+041 & \cite{Whysong2004}  \\
        2.80E+13 & 1.51E+041 & \cite{Perlman2001}  \\
        2.47E+14 & 1.28E+041 & \cite{Prieto2016}   \\
        3.32E+14 & 1.39E+041 & \cite{Prieto2016}   \\
        3.70E+14 & 7.55E+040 & \cite{Prieto2016}   \\
        4.99E+14 & 6.81E+040 & \cite{Prieto2016}   \\
        6.32E+14 & 8.40E+040 & \cite{Prieto2016}   \\
        8.93E+14 & 5.15E+040 & \cite{Prieto2016}   \\
        1.10E+15 & 4.53E+040 & \cite{Prieto2016}   \\
        1.27E+15 & 7.40E+040 & \cite{Prieto2016}   \\
        1.36E+15 & 4.73E+040 & \cite{Prieto2016}   \\
        2.06E+15 & 2.75E+040 & \cite{Prieto2016}   \\
        2.42E+17 & 1.95E+040 & \cite{Prieto2016}   \\
        2.42E+18 & 1.79E+040 & \cite{Prieto2016}   \\
        \hline
    \end{tabular}
    \caption{SED data for M87.}
    \label{tab:M87}
\end{table}



\begin{table}
    \centering
    \begin{tabular}{lcc}
        \hline
        $\nu$ (Hz) & $\nu L_{\nu}$ (erg s$^{-1}$) & Reference \\
        \hline
        1.40E+09  & 2.86E+39  & \cite{Capetti2005} \\
        2.50E+09  & 5.28E+39  & \cite{Lazio2001}\\
        5.00E+09  & 9.11E+39 & \cite{Nagar2005}\\
        1.50E+10 & 3.68E+40 & \cite{Nagar2005} \\
        8.62E+10 & ($2.28\pm0.13$)E+41 & \cite{Agudo2014} \\
        2.29E+11 & ($3.08\pm0.23$)E+41 & \cite{Agudo2014} \\
        3.75E+13 & ($1.47\pm0.08$)E+42 & \cite{Gu2007} \\
        5.17E+13 & ($7.72\pm0.59$)E+41 & \cite{Gu2007} \\
        6.67E+13 & ($4.63\pm0.45$)E+41 & \cite{Gu2007} \\
        8.33E+13 & ($2.95\pm0.35$)E+41 & \cite{Gu2007} \\
        3.68E+14 & 2.00E+41 & \cite{VerdoesKleijn2002} \\
        5.40E+14 & 9.48E+40 & \cite{VerdoesKleijn2002} \\ 
        (4.8--24)E+17 & 4.36E+41 & \cite{Gonzalez-Martin2006} \\   
        \hline
    \end{tabular}
    \caption{SED data for NGC 315.}
    \label{tab:NGC315}
\end{table}




\begin{table}
    \centering
    \begin{tabular}{lcc}
        \hline
        $\nu$ (Hz) & $\nu L_{\nu}$ (erg s$^{-1}$) & Reference \\
        \hline
        1.63E+09 & 2.40E+38 & \cite{Jones1997} \\
        5.00E+09 & 5.88E+38 & \cite{Nagar2005} \\
        8.39E+09 & 1.24E+39 & \cite{Jones1997} \\
        1.50E+10 & 6.71E+39 & \cite{Nagar2005} \\
        1.66E+13 & ($5.39\pm0.24$)E+41 & \cite{Asmus2014} \\
        2.50E+13 & ($4.79\pm1.10$)E+41 & \cite{Asmus2014} \\
        3.64E+14 & > 6.03E+39 & \cite{Ferrarese1996} \\
        4.41E+14 & > 4.60E+39 & \cite{Ferrarese1996} \\
        5.41E+14 & > 3.96E+39 & \cite{Ferrarese1996} \\
        (4.8--24)E+17 & 1.03E+41 &  \cite{Zezas2005} \\
        \hline
    \end{tabular}
    \caption{SED data for NGC 4261.}
    \label{tab:NGC4261}
\end{table}
